Learning to Drive on the Wrong Side of the Road: How American Computing Came to Rely on Conferences for Primary Publication

In contrast to other fields where conferences are typically for less polished or in-progress research, computing has long relied on referred conference papers as a venue for the final publication of completed research. While frequently a topic of informal discussion, debates about its efficacy, or library science research, the development of this phenomena has not been historically analyzed. This paper presents the first systematic investigation of the development of modern computing publications. It relies on semi-structured interviews with eight computing professors from diverse backgrounds to understand how researchers experienced changes in publication culture over time. Ultimately, the article concludes that the early presence of non-academic practitioners in research and a degree of "path dependence"or a tendency to continue on the established path rather than the most economically optimal one" allowed conferences to gain and hold prominence as the field exploded in popularity during the 1980s.

==> frontmatter/abstract.tex <==
\chapter*{Abstract}
In contrast to other fields where conferences are typically for less polished or in-progress research, computing has long relied on referred conference papers as a venue for the final publication of completed research. While frequently a topic of informal discussion, debates about its efficacy, or library science research, the development of this phenomena has not been historically analyzed. This paper presents the first systematic investigation of the development of modern computing publications. It relies on semi-structured interviews with eight computing professors from diverse backgrounds to understand how researchers experienced changes in publication culture over time. Ultimately, the article concludes that the early presence of non-academic practitioners in research and a degree of "path dependence"—or a tendency to continue on the established path rather than the most economically optimal one—allowed conferences to gain and hold prominence as the field exploded in popularity during the 1980s. 

==> frontmatter/copyright.tex <==
\cleardoublepage

\noindent Copyright \textcopyright\ 2018 by [Author's Name]

\noindent All rights reserved

\thispagestyle{empty}
\cleardoublepage


==> frontmatter/dedication.tex <==
\cleardoublepage
\begin{center}
	\vspace*{\stretch{1}}
	
	To [Name]
	
	\vspace*{\stretch{2}}
\end{center}
\cleardoublepage

